A Secure Distributed Authentication scheme based on CRT-VSS and Trusted Computing in MANET

With the rapid development of MANET, secure and practical authentication is becoming increasingly important. The existing works perform the research from two aspects, i.e., (a)secure key division and distributed storage, (b)secure distributed authentication. But there still exist several unsolved problems. Specifically, it may suffer from cheating problems and fault authentication attack, which can result in authentication failure and DoS attack towards authentication service. Besides, most existing schemes are not with satisfactory efficiency due to exponential arithmetic based on Shamir's scheme. In this paper, we explore the property of verifiable secret sharing(VSS) schemes with Chinese Remainder Theorem (CRT), then propose a secret key distributed storage scheme based on CRT-VSS and trusted computing for MANET. Specifically, we utilize trusted computing technology to solve two existing cheating problems in secret sharing area before. After that, we do the analysis of homomorphism property with CRT-VSS and design the corresponding shares-product sharing scheme with better concision. On such basis, a secure distributed Elliptic Curve-Digital Signature Standard signature (ECC-DSS) authentication scheme based on CRT-VSS scheme and trusted computing is proposed. Furthermore, as an important property of authentication scheme, we discuss the refreshing property of CRT-VSS and do thorough comparisons with Shamir's scheme. Finally, we provide formal guarantees towards our schemes proposed in this paper.

==> homomorphism.tex <==
\subsection{distributed authentication}
%In order to tolerate mobile adversaries, the key management service proposed in \cite{LidongZhou} employs share refreshing as an important scheme which relying on the $(\oplus,\oplus)$ homomorphism property. It is indicated in \cite{homomorphisms} that the traditional Shamir's threshold scheme only has the $(\oplus,\oplus)$-homomorphism property, without the $(\otimes,\otimes)$ or $(\oplus,\otimes)$- property. While it's only mentioned in \cite{homomorphisms},\cite{Iftene} that the extended Asmuth-Bloom scheme has homomorphism proprieties but without any proof about it. The discussion about the homomorphism property of the CRT-VSS scheme is rare.


In the Distributed CA scheme in \cite{LidongZhou}, the private key of CA is divided into several shares and distributed to several chosen entities, and each has one and only one part. Distributed authentication is the result of the Distributed CA scheme in the distributed environment of MANET. The scheme proposed in \cite{xiongyan} realize the authentication with the process of the multi-hop signing. The encrypted  functions mechanism\cite{Encryptedfunction} is used to strengthen the privacy and security of the authentication process, similar related work can be seen in \cite{ertaul2005security}. In \cite{gennaro1996robust}, a meaningful robust DSS signature schemes are proposed under  different security requirements.
But in all the schemes proposed above, the choice of nodes coalition for authentication is random and  lacks  validation, including the secret shares and the trusted property of the nodes. This may lead to DoS  and fault attack problem  \cite{faultattack2010} . Besides, RSA/Elgamal  encrypt/decrypt  and signature mechanism  utilized by all the schemes above has a relative limited efficiency in MANET according to analysis in \cite{ertaul2005security}.


